Provably Robust Deep Learning via Adversarially Trained Smoothed Classifiers

Recent works have shown the effectiveness of randomized smoothing as a scalable technique for building neural network-based classifiers that are provably robust to $\ell_2$-norm adversarial perturbations. In this paper, we employ adversarial training to improve the performance of randomized smoothing. We design an adapted attack for smoothed classifiers, and we show how this attack can be used in an adversarial training setting to boost the provable robustness of smoothed classifiers. We demonstrate through extensive experimentation that our method consistently outperforms all existing provably $\ell_2$-robust classifiers by a significant margin on ImageNet and CIFAR-10, establishing the state-of-the-art for provable $\ell_2$-defenses. Moreover, we find that pre-training and semi-supervised learning boost adversarially trained smoothed classifiers even further. Our code and trained models are available at http://github.com/Hadisalman/smoothing-adversarial .

==> deprecated.tex <==
% We employ projected gradient descent (PGD) \citep{madry2017towards} to attack randomized smoothing classifiers. Note that the smoothed classifier is not a neural network, and in fact is not a differentiable function.\jerry{Not true, it is differentiable} A smoothed classifier, as previously mentioned in Section~\ref{sec:randomized-smoothing}, constitutes of a base classifier $f$ (in practice a neural network) that maps an input $x \in \mathbb{R}$ to classes $\mathcal Y$. The smoothed classifier $g$ is then defined as in \eqref{g}. Assume that for a given input $\bar{x}$, the true class is $c^*$. Then in order to fool $g$, an adversary must find an adversarial example $\hat{x}$ in the neighborhood of x such that,
% \begin{align}
% \hat{x} &= \argmin_{x \in\mathcal{B}_\epsilon(\bar{x})} \mathbb{P}_{\delta \sim \mathcal{N}(0, \sigma^2 I)} (f(x+\delta) = c^*)
% \end{align}
% where $\mathcal{B}_\epsilon(\bar{x})$ is an $\ell_2$-normed ball of radius $\epsilon$ centered at $\bar{x}$. \seb{I reiterate that to me it is more natural to consider the convolution with a Gaussian of the distribution obtained by the logit. Minimizing the classical cross-entropy loss of that object is exactly equivalent to \eqref{eq:pgd-attack}. My suggestion is to derive the latter equation with this argument, and then use the current one as an alternative justification.} Note that this objective function is clearly not differentiable, therefore we approximate with a differentiable function as follows,
% \begin{align}
% \hat{x} &=\argmin_{x \in\mathcal{B}_\epsilon(\bar{x})} \mathbb E_{\delta \sim \mathcal{N}(0, \sigma^2 I)} \left[\mathbb I(f(x+\delta) = c^*)\right]\\\nonumber
% \hat{x} &\approx \argmin_{x \in\mathcal{B}_\epsilon(\bar{x})} \mathbb E_{\delta \sim \mathcal{N}(0, \sigma^2 I)} \left[softmax\left(\eta f_{logit}(x+\delta)\right)_{c^*}\right]
% \end{align}
% where $f_{logit} \in \mathbb R^{| \mathcal{Y}|}$ is the logit layer of the base neural network $f$, and $\eta$ is a hyper-parameter (\textit{temperature}) that can tuned to allow the softmax to approximate the indicator function arbitrarily close. For neural network optimization, it is usually better to optimize the log probabilities instead of directly optimizing probabilities (better numerical stability and avoiding vanishing gradients). Therefore  finding an adversarial examples simplifies to solving the following optimization problem,
% \begin{align}\label{eq:pgd-attack}
% \hat{x} &\approx \argmin_{x \in\mathcal{B}_\epsilon(\bar{x})} \log\mathbb E_{\delta \sim \mathcal{N}(0, \sigma^2 I)} \left[softmax\left(\eta f_{logit}(x+\delta)\right)_{c^*}\right]
% \end{align}
% % We note that \eqref{eq:pgd-attack} should not be confused with 
% % \begin{align}\label{eq:wrong-attack}
% % \hat{x} &= \argmin_{x \in\mathcal{B}_\epsilon(\bar{x})} \mathbb E_{\delta \sim \mathcal{N}(0, \sigma^2 I)} \left[\log softmax\left(\eta f_{logit}(x+\delta)\right)_{c^*}\right]\\\nonumber
% % &= \argmin_{x \in\mathcal{B}_\epsilon(\bar{x})} \mathbb E_{\delta \sim \mathcal{N}(0, \sigma^2 I)} \left[\ell (f_{logits}(x+\delta), c^*)\right]
% % \end{align}
% % where $\ell$ is the cross entropy loss, as suggested in section G.3 of \cite{cohen2019certified}. \textit{There is a key subtlety between \eqref{eq:pgd-attack} and \eqref{eq:wrong-attack}; conceptually, \eqref{eq:wrong-attack} is basically finding an adversarial example of $f$ that is robust to gaussian noise, where as \eqref{eq:pgd-attack} is actually attacking the right model i.e. trying  to find adversarial examples that decreases the probability of correct classification of the smoothed classifier $g$. Therefore \eqref{eq:pgd-attack} is the right optimization problem that should be used to find adversarial examples of $g$.} \seb{This paragraph is very important, and I would suggest to allude to it much earlier. Maybe in the paragraph on our contribution, by saying that there is a subtlety/ambiguity on how to find good adversarial examples for a smoothed classifier, which we resolve.}

% The formulation in \eqref{eq:wrong-attack} was also mentioned in section G.3 of \cite{cohen2019certified} as one \textit{naive} attack that, although able to find some adversarial examples to the $g$, is ``not actually the objective of interest'', i.e. is \textit{not} attacking the smoothed classifier $g$.

% The optimization problem \eqref{eq:pgd-attack} can be solved using PGD and using your favorite autodiff library. \seb{I assume we are gonna say more about the gradient, how we approximate it, etc? Or maybe that's supposed to be Section 5?}
